Grant-Free Random Access of IoT devices in Massive MIMO with Partial CSI

The number of wireless devices is drastically increasing, resulting in many devices contending for radio resources. In this work, we present an algorithm to detect active devices for unsourced random access, i.e., the devices are uncoordinated. The devices use a unique, but non-orthogonal preamble, known to the network, prior to sending the payload data. They do not employ any carrier sensing technique and blindly transmit the preamble and data. To detect the active users, we exploit partial channel state information (CSI), which could have been obtained through a previous channel estimate. For static devices, e.g., Internet of Things nodes, it is shown that CSI is less time-variant than assumed in many theoretical works. The presented iterative algorithm uses a maximum likelihood approach to estimate both the activity and a potential phase offset of each known device. The convergence of the proposed algorithm is evaluated. The performance in terms of probability of miss detection and false alarm is assessed for different qualities of partial CSI and different signal-to-noise ratio.

==> Section/Channel_Estimation_Decoding.tex <==
\section{Channel estimation and Payload Decoding}
After the activity detection phase, the transmitted preambles can be used to estimate the channel. Hereafter, the payload can be decoded based on the channel estimate. 


\subsection{Received Preambles and Payload}
The received preamble symbols at the receive antennas are modeled as,
\begin{align}
     \mat{Y}_p =  \mat{H}_a  \mat{S}_a +  \mat{W}_p\in \mathbb{C}^{M\times T_p}.
\end{align}
The transmitted preamble with length $T_p$, of the $K_a=|\mathcal{K}_a|$ active users, is denoted by $\mat{S}_a \in~\mathbb{C}^{K_a\times T_p}$. \gilles{do we need to explain $W_p$ and $W_d$?}

After transmitting the preamble, the active users sent their payload data. The received payload symbols are given by
\begin{align}
     \mat{Y}_d =  \mat{H}_a  \mat{X} +  \mat{W}_d\in \mathbb{C}^{M\times T_d},
\end{align}
with $\mat{X}\in \mathbb{C}^{K_a \times T_d}$ the payload symbols from the $K_a$ devices.

\subsection{Channel Estimation}
\gilles{change variable name $S_a$ is it is here the detected active users, not actually the active users. Maybe $S_{ad}$}
Based on the thresholding described in Section~\ref{section:Device_Activity_Detection}, the user activity is determined. Let $\mat{S}_{ad} \in \mathbb{C}^{K_{ad}\times T_p}$ be the preamble symbols of the considered $K_{ad}=|\mathcal{K}_{ad}|$ active users.

\gilles{have to change subscript a to ad}
Using part of the \gls{csi} as modeled in (\ref{eq:prior_CSI_channel_model}), we can write the received preamble signals as,
\begin{align}
     \mat{Y}_p =  \left(\mat{G}_a + \mat{E}_a\right) \mat{S}_a \diag\left(\vect{\gamma}\right) +  \mat{W}_p.
\end{align}
In the device activity phase, $\vect{\gamma}$ is estimated, and $\mat{G}_a$ and $\mat{S}_a$ are known. From this $\mat{E}_a$ can be estimated based on the pseudo-inverse, whereafter the channel estimate can be obtained. 
\begin{align}
     \mat{Y}_p - \mat{G}_a \mat{S}_a =  \mat{E}_a \diag\left(\vect{\gamma}\right) \mat{S}_a 
\end{align}

\begin{align}
     \mat{E}_a \diag\left(\vect{\gamma}\right) &= (\mat{Y}_p - \mat{G}_a \mat{S}_a) \mat{S}_a^{\dagger}\\
     \mat{E}_a &= (\mat{Y}_p - \mat{G}_a \mat{S}_a) \mat{S}_a^{\dagger} \diag\left(\vect{\gamma}\right)^{-1}
\end{align}

The channel estmate is then computed as,
\begin{align}
     \hat{\mat{H}}_a =  \mat{G}_a + \mat{E}_a.
\end{align}


% The channel can be estimated through the \gls{ls} method~\cite{kay1993fundamentals}, by using the right pseudo-inverse of the preambles,
% \begin{align}
%     \hat{\mat{H}}_{ad}&= \mat{Y}_p \mat{S}^H_{ad} \left(\mat{S}_{ad} \mat{S}_{ad}^H\right)^{-1} \in \mathbb{C}^{M\times K_{ad}},
% \end{align}
% with $\mat{Y}_p \in \mathbb{C}^{M\times T_p}$ the received preamble symbols. Note that the \gls{ls} is the same as the \gls{ml} estimator if the noise is Gaussian, which is here the case. Using \gls{ls} assumes that $\mat{S}_{ad}$ is full rank, thereby guarantying the invertibility of $\left(\mat{S}_{ad} \mat{S}_{ad}^H\right)$. This requires that $|\mathcal{K}_{ad}| \leq T_p$ and that $M$ is sufficiently large enough in order to have uncorrelated \gls{iid} preambles. 

\subsection{Payload decoding}
Once the channels are estimated, the payload data of the $K_{ad}$ devices can be decoded with the conventional methods. Again, the \gls{zf} approach can be applied using the decoder matrix,
\begin{align}
    \mat{W} &= \left(\hat{\mat{H}}_{ad}^H \hat{\mat{H}}_{ad}\right)^{-1} \hat{\mat{H}}_{ad}^H \in \mathbb{C}^{K_{ad} \times M}.
\end{align}
% The decoder is normalized to have unit power, i.e., $\alpha = 1/||W||^2$. Note that the matrix normalization does not give equal power to each user. 
The payload can then be decoded by applying the decoder matrix on the received symbols,
\begin{align}
    \hat{\mat{X}}_{ad} &= \mat{W} \mat{Y}_d \in \mathbb{C}^{K_{ad} \times T_d},
\end{align}
with $\mat{Y}_d \in \mathbb{C}^{M \times T_d}$ the received payload data of $T_d$ symbols. Note the subscript $ad$ denoting that $\hat{\mat{X}}_{ad}$ contains the payload symbols of the considered active devices. 



==> rev/before-pruning-for-wcnc/Section/Channel_Estimation_Decoding.tex <==
\section{Channel estimation and Payload Decoding}
After the activity detection phase, the transmitted preambles can be used to estimate the channel. Hereafter, the payload can be decoded based on the channel estimate. 


\subsection{Received Preambles and Payload}
The received preamble symbols at the receive antennas are modeled as,
\begin{align}
     \mat{Y}_p =  \mat{H}_a  \mat{S}_a +  \mat{W}_p\in \mathbb{C}^{M\times T_p}.
\end{align}
The transmitted preamble with length $T_p$, of the $K_a=|\mathcal{K}_a|$ active users, is denoted by $\mat{S}_a \in~\mathbb{C}^{K_a\times T_p}$. \gilles{do we need to explain $W_p$ and $W_d$?}

After transmitting the preamble, the active users sent their payload data. The received payload symbols are given by
\begin{align}
     \mat{Y}_d =  \mat{H}_a  \mat{X} +  \mat{W}_d\in \mathbb{C}^{M\times T_d},
\end{align}
with $\mat{X}\in \mathbb{C}^{K_a \times T_d}$ the payload symbols from the $K_a$ devices.

\subsection{Channel Estimation}
\gilles{change variable name $S_a$ is it is here the detected active users, not actually the active users. Maybe $S_{ad}$}
Based on the thresholding described in Section~\ref{section:Device_Activity_Detection}, the user activity is determined. Let $\mat{S}_{ad} \in \mathbb{C}^{K_{ad}\times T_p}$ be the preamble symbols of the considered $K_{ad}=|\mathcal{K}_{ad}|$ active users.

\gilles{have to change subscript a to ad}
Using part of the \gls{csi} as modeled in (\ref{eq:prior_CSI_channel_model}), we can write the received preamble signals as,
\begin{align}
     \mat{Y}_p =  \left(\mat{G}_a + \mat{E}_a\right) \mat{S}_a \diag\left(\vect{\gamma}\right) +  \mat{W}_p.
\end{align}
In the device activity phase, $\vect{\gamma}$ is estimated, and $\mat{G}_a$ and $\mat{S}_a$ are known. From this $\mat{E}_a$ can be estimated based on the pseudo-inverse, whereafter the channel estimate can be obtained. 
\begin{align}
     \mat{Y}_p - \mat{G}_a \mat{S}_a =  \mat{E}_a \diag\left(\vect{\gamma}\right) \mat{S}_a 
\end{align}

\begin{align}
     \mat{E}_a \diag\left(\vect{\gamma}\right) &= (\mat{Y}_p - \mat{G}_a \mat{S}_a) \mat{S}_a^{\dagger}\\
     \mat{E}_a &= (\mat{Y}_p - \mat{G}_a \mat{S}_a) \mat{S}_a^{\dagger} \diag\left(\vect{\gamma}\right)^{-1}
\end{align}

The channel estmate is then computed as,
\begin{align}
     \hat{\mat{H}}_a =  \mat{G}_a + \mat{E}_a.
\end{align}


% The channel can be estimated through the \gls{ls} method~\cite{kay1993fundamentals}, by using the right pseudo-inverse of the preambles,
% \begin{align}
%     \hat{\mat{H}}_{ad}&= \mat{Y}_p \mat{S}^H_{ad} \left(\mat{S}_{ad} \mat{S}_{ad}^H\right)^{-1} \in \mathbb{C}^{M\times K_{ad}},
% \end{align}
% with $\mat{Y}_p \in \mathbb{C}^{M\times T_p}$ the received preamble symbols. Note that the \gls{ls} is the same as the \gls{ml} estimator if the noise is Gaussian, which is here the case. Using \gls{ls} assumes that $\mat{S}_{ad}$ is full rank, thereby guarantying the invertibility of $\left(\mat{S}_{ad} \mat{S}_{ad}^H\right)$. This requires that $|\mathcal{K}_{ad}| \leq T_p$ and that $M$ is sufficiently large enough in order to have uncorrelated \gls{iid} preambles. 

\subsection{Payload decoding}
Once the channels are estimated, the payload data of the $K_{ad}$ devices can be decoded with the conventional methods. Again, the \gls{zf} approach can be applied using the decoder matrix,
\begin{align}
    \mat{W} &= \left(\hat{\mat{H}}_{ad}^H \hat{\mat{H}}_{ad}\right)^{-1} \hat{\mat{H}}_{ad}^H \in \mathbb{C}^{K_{ad} \times M}.
\end{align}
% The decoder is normalized to have unit power, i.e., $\alpha = 1/||W||^2$. Note that the matrix normalization does not give equal power to each user. 
The payload can then be decoded by applying the decoder matrix on the received symbols,
\begin{align}
    \hat{\mat{X}}_{ad} &= \mat{W} \mat{Y}_d \in \mathbb{C}^{K_{ad} \times T_d},
\end{align}
with $\mat{Y}_d \in \mathbb{C}^{M \times T_d}$ the received payload data of $T_d$ symbols. Note the subscript $ad$ denoting that $\hat{\mat{X}}_{ad}$ contains the payload symbols of the considered active devices. 



==> rev/before-pruning-for-wcnc/Section/Conclusion.tex <==
\section{Conclusion}\label{section:conclusion}
\glsresetall % reset glossaries for those reading only the conclusion

We formulated an iterative \gls{ml} algorithm to detect active devices using prior \gls{csi} when performing grant-free random access. Previous experimental work has demonstrated that, in many \gls{mmtc} applications, the \gls{csi} is less time-variant than assumed in theoretical models. Given the static nature of \gls{iot} devices, we have exploited this feature in the activity detection estimator. During grant-free access, the devices transmit a unique, but non-orthogonal preamble, which is used for activity detection. Next to this, the algorithm is also able to detect a device-specific phase offset, which could be caused by \gls{cfo}. The algorithm is numerically evaluated and compared to the conventional \gls{lmmse} estimator with full channel knowledge and partial \gls{csi}. The presented results indicate that the iterative algorithm converges and outperforms the conventional \gls{lmmse} estimator. For a \gls{snr} of \SI{6.67}{\deci\bel}, the probability of not detecting an active device is \num{21} times lower for the proposed iterative \gls{ml} estimator than the \gls{lmmse} estimator for the same probability of wrongly considering an inactive device as an active device.

This work can be extended to the cell-free or distributed case with geographically distributed access points. In that case, the partial \gls{csi} becomes access point-dependent.


==> rev/before-pruning-for-wcnc/Section/Device_Activity_Detection.tex <==
\section{Device Activity Detection}%
\label{section:Device_Activity_Detection}

This section describes the proposed activity detection algorithm. First, the log-likelihood of the received preamble is derived. Then, given its non-convex expression, an iterative approach is proposed to estimate the parameters $\gamma_k\ \forall k$. Finally, activity detection is performed.

\subsection{Log-Likelihood of the Received Symbols}

Combining (\ref{eq:received_symbol}) and (\ref{eq:prior_CSI_channel_model}), the symbol, received at \gls{bs} antenna $m$ and for pilot symbol $t$, is given by
\begin{align*}
	y_{t,m}&=\sum_{k=0}^{K-1} ({g}_{k,m} + {\epsilon}_{k,m} \lambda_k  )  s_{t,k} \gamma_k + {w}_{t,m}.
\end{align*}
Stacking the observations at antenna $m$ gives
\begin{align*}
\vect{y}_{m}&=\sum_{k=0}^{K-1} {g}_{k,m} \vect{s}_{k} \gamma_k + \sum_{k=0}^{K-1} {\epsilon}_{k,m} \lambda_k  \vect{s}_{k} \gamma_k  + \vect{w}_{m},
\end{align*}
where
\begin{align*}
    \vect{y}_m&=\begin{pmatrix} y_{0,m}\\ \vdots \\ y_{T-1,m} \end{pmatrix},\ \vect{s}_k=\begin{pmatrix} s_{0,k}\\ \vdots \\ s_{T-1,k} \end{pmatrix},\ \vect{w}_m=\begin{pmatrix} w_{m,0}\\ \vdots \\ w_{T-1,m} \end{pmatrix}.
\end{align*}
For a given value of $\gamma_k$, $\vect{y}_{m}|\gamma_k$ has a circularly symmetric Gaussian distribution with mean $\sum_{k=0}^{K-1} {g}_{k,m} \vect{s}_{k} \gamma_k $. After defining the vector $
\vect{\theta}_m =\sum_{k=0}^{K-1} {\epsilon}_{k,m} \lambda_k  \vect{s}_{k} \gamma_k  + \vect{w}_{m}$, the covariance matrix is
\begin{align}\label{eq:covariance_matrix_C}
\mat{C}&=\mathbb{E}\left( \vect{\theta}_m \vect{\theta}^H_m\right)\\
 &=\sum_{k=0}^{K-1}\lambda_k^2|\gamma_k|^2 \vect{s}_k\vect{s}_k^H +\sigma^2\mat{I}_T, 
\end{align}
where we used the fact that ${\epsilon}_{k,m}$ were assumed to be \gls{iid} and the additive noise is white. Note that this covariance matrix does not depend on the antenna index $m$ and is thus valid for all $\vect{y}_m$.
% \begin{align*}
% \mat{C}&= \mathbb{E}(| \vect{y}_{m}- \mathbb{E}(\vect{y}_{m})|^2)\\
% &= \mathbb{E}\left(\left|\sum_{k=0}^{K-1} {g}_{k,m} \vect{s}_{k} \gamma_k + {\epsilon}_{k,m} \lambda_k  \vect{s}_{k} \gamma_k  + \vect{w}_{m} - \sum_{k=0}^{K-1} {g}_{k,m} \vect{s}_{k} \gamma_k\right|^2\right )\\
% &= \mathbb{E}\left(\left|{\epsilon}_{k,m} \lambda_k  \vect{s}_{k} \gamma_k  + \vect{w}_{m}\right|^2 \right)\\
% &= \mathbb{E}\left(\left({\epsilon}_{k,m} \lambda_k  \vect{s}_{k} \gamma_k  + \vect{w}_{m}\right)
% \left({\epsilon}_{k,m} \lambda_k  \vect{s}_{k} \gamma_k  + \vect{w}_{m}\right)^H
% \right)\\
% \end{align*}
Defining the vector $\vect{\gamma}=(\gamma_0,...,\gamma_{K-1})^T$, and $\vect{\Theta}_m=\vect{y}_m - \sum^{K-1}_{k=0} g_{k,m} \vect{s}_{k} \gamma_k$ the log-likelihood of the observation vector $\vect{y}_m$ is
\begin{align*}
\log p(\vect{y}_{m}|\vect{\gamma})&=-\ln\left(\left|\mat{C}\right|\right)-T\ln(\pi)
-\vect{\Theta}_m^H
\mat{C}^{-1} \vect{\Theta}_m.
\end{align*}
Given the conditional independence of ${\epsilon}_{k,m}$ and ${w}_{t,m}$ over the antennas, the different $\vect{y}_m$ are independent as well. Hence, the log-likelihood of the aggregated observations at all antennas $\vect{y}=(\vect{y}_0^T,...,\vect{y}_{M-1}^T)^T$ becomes 
\begin{align}
&\log p(\vect{y}|\vect{\gamma})=\sum_{m=0}^{M-1} \log p(\vect{y}_m|\vect{\gamma})\label{eq:log_likelihood}\\
&=-M\ln\left(\left|\mat{C}\right|\right)-MT\ln(\pi)-\sum_{m=0}^{M-1}\vect{\Theta}_m^H
\mat{C}^{-1}
\vect{\Theta}_m\nonumber.%\\
% &=-M\ln\left(\left|\mat{C}\right|\right)-MT\ln(\pi)-\sum_{m=0}^{M-1}\left(\vect{y}_{m}-\mat{\Gamma}_m \vect{\gamma}\right)^H
% \mat{C}^{-1}
% \left(\vect{y}_{m}-\mat{\Gamma}_m \vect{\gamma}\right),
\end{align}
% where we defined
% \begin{align*}
% 	\mat{\Gamma}_m&=\begin{pmatrix}
% 	\vect{s}_0 & ... & \vect{s}_{K-1}
% 	\end{pmatrix}\diag(g_{m,0},...,g_{k,m-1}).
% %	\mat{Y}&=\begin{pmatrix}
% %	\vect{y}_0 & ... & \vect{y}_{M-1}
% %	\end{pmatrix}
% \end{align*}


% One of the difference with the approaches in \cite{GanesanTCOM,FenglerTIT} is that we consider complex coefficients $\gamma_k$ and not simply real. This changes the optimization procedure and I am not sure we can use their simple trick... Another main difference is that we do not have just $\vect{y}_m$ but $\vect{y}_m$ minus something that depends on $\gamma_k$.

\subsection{Iterative Algorithm for Maximizing Likelihood}

The maximum likelihood estimator of $\vect{\gamma}$ is obtained by maximizing
\begin{align*}
    \hat{\vect{\gamma}}_{\mathrm{ML}} &= \arg \max_{\vect{\gamma}} \log p(\vect{y}|\vect{\gamma}).
\end{align*}
This problem is not trivial to solve given the nonlinear and non-convex dependence of the log-likelihood, more specifically the covariance matrix $\mat{C}$, in $\vect{\gamma}$. 
An idea to maximize the likelihood is to use an iterative approach, similarly as \cite{GanesanTCOM,FenglerTIT}: at each iteration, all $\gamma_k$ are kept fixed but one, which is optimized and updated. This way, they get updated one by one until convergence is attained, \textit{i.e.}, a maximum number of iterations or a certain tolerance is reached. A block diagram of the algorithm is given in Figure~\ref{fig:iterative_algorithm} and the pseudocode is summarized in Algorithm~\ref{alg:cap}.

% \begin{figure}[t!]
% 	\centering 
% 	\resizebox{0.8\linewidth}{!}{%
% 		{\includegraphics[clip, trim=0cm 8.5cm 12.5cm 0cm, scale=1]{Fig/iterative_algorithm.pdf}} %gauche bas droite haut
% 	}
	
% 	\caption{Block diagram of the iterative maximum likelihood estimator and activity detection.\TODO{add cross refs to equation numbers for the optimizations}}\label{fig:iterative_algorithm} 
% 	\vspace{-1em}
% \end{figure}


\begin{figure*}[t!]
	\centering 
\resizebox{.7\textwidth}{!}{%

\tikzstyle{block} = [draw, rectangle, 
    minimum height=3em, minimum width=6em, minimum height = 3em, minimum width = 10em]
\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{container} = [draw, rectangle, inner sep=0.4cm]
\tikzstyle{decision} = [diamond, draw, text badly centered, inner sep=3pt]


\begin{tikzpicture}[auto, node distance=1.5cm,>=latex']

    % We start by placing the blocks
    \node [block, name=input, align=center, font=\large] (input) {\large Inputs\\ $\sigma^2$, $\lambda_k$, $g_{m,k}$,\\ $\vect{y}_m$ $\forall m,k$ \\ 
    Initialization \\ $k' \gets 0$, $\hat{\vect{\gamma}} \gets \hat{\vect{\gamma}}_{\mathrm{init}}$};
    

    

    \node [block, minimum height = 6em, minimum width=16em, align=center, right= of input, font=\large] (amplitude) {\large Amplitude   Optimization\\ (\ref{eq:update_partial_CSI}), (\ref{eq:update_no_CSI}) or (\ref{eq:update_prior_CSI}) \\ $\hat{r}_{k'} \gets \arg \max \tilde{f}(r_{k'})$};
    
    \node [block, align=center, minimum height = 6em, minimum width=16em, right= of amplitude, font=\large] (phase) {\large Phase  Optimization~(\ref{eq:phase_update})\\  $\hat{\phi}_{k'} \gets \angle  \vect{s}_{k'}^H \mat{C}^{-1} \sum_{m=0}^{M-1} {g}_{k',m}^*  \vect{y}_{k',m}$};
    
    
    %\path (amplitude) -- (phase) coordinate[midway] (aux);
    
    %\node [block, align=center, below of=aux] (update) {Update\\ $\hat{\gamma}_k = \hat{r}_{k'} e^{\jmath\phi_{k'}} $};

   \node [container,fit=(amplitude) (phase), label=below:{}, dashed] (inner_container) {};
   
  
   \node [decision, below=of inner_container] (converged) {Converged?};
   
   %\node [block, align=center, left= of converged] (iter) {$k' \gets k'+1 \mod K$};
    
   \node [container,fit=(converged) (inner_container), label=above:{\large Iterative maximum likelihood estimator}] (outer_container) {};

   
   \node [block, name=tolerance, align=center, left=of converged.center, below=2.8cm of input, font=\large, anchor=center] (tolerance) {\large Tolerance \\ Max iteration};

    \node [block, align=center, below=of converged, font=\large] (detection) {\large Activity Detection\\ $\hat{\gamma}_k \leq  \gamma_{th,k}\ \forall k$};
    
    
    \draw[->] (input.east) -- (inner_container.west);
    %\draw[->] (init.east) |- (inner_container.west);
    
    \draw[->] (tolerance.east) -- (converged.west);
    
    %\draw[->] (converged.west) -- node[midway]{No} (iter.east);
    

    \node [] at ([shift={(0.3,0.3)}]converged.east) {No};
    
    \node [] at ([shift={(0.4,-0.1)}]converged.south) {Yes};
    
    
    \draw[->] (converged.east) -|node[below, font=\large]{$k' \gets k'+1 \mod K$} (inner_container.-20);
    
     %\draw[->] (iter.north) -- (amplitude.south);
     
     \draw[->] (inner_container.south) --node[left, font=\large]{Updated $\hat{\gamma}_{k'} \gets \hat{r}_{k'} e^{\jmath\phi_{k'}} $} (converged.north);
    
    \draw[->] (converged.south) --node[near end]{$\hat{\vect{\gamma}}$} (detection.north);
    
\end{tikzpicture}%
}

	\caption{Block diagram of the iterative maximum likelihood estimator and activity detection.}\label{fig:iterative_algorithm} 
	%\vspace{-1em}
\end{figure*}


Let us consider that the complex-valued $\gamma_{k'}$ needs to be updated. Using the definition introduced in (\ref{eq:definition_gamma_k}), we can rewrite $\gamma_{k'}$ with a phase-amplitude decomposition: $\gamma_{k'}=r_{k'}e^{\jmath\phi_{k'}}$, with $r_{k'}=|\gamma_{k'}|=\sqrt{\rho_{k'}}a_{k'}$. The optimization with respect to $\gamma_{k'}$ is done in the following in several steps: i)~optimizing the phase $\phi_{k'}$ for a fixed value of $r_{k'}$, ii)~re-inserting this expression in the objective function to remove the dependence in~$\phi_{k'}$ and iii)~optimizing the amplitude $r_{k'}$. 

\subsubsection{Phase optimization}

To highlight the dependence of the objective function in $\gamma_{k'}$ for constant values of other~$\gamma_{k},\ k\neq k'$, let us define the vector
\begin{align}
	\vect{y}_{k',m}&=\vect{y}_{m}-\sum_{k=0, k\neq k'}^{K-1} {g}_{k,m} \vect{s}_{k} \gamma_k, \label{eq:y_m_k_prime}
\end{align}
which can be seen as a cancellation of device interference to isolate the contribution from device~$k'$. Hence, the objective function to maximize can be written as\footnote{For clarity, we omit in the following the constant term $MT\ln(\pi)$ which does not affect optimization as it does not depend on $\vect{\gamma}$ and vanishes after differentiation.}
\begin{align*}
f(r_{k'},\phi_{k'})&=-M\ln\left(\left|\mat{C}\right|\right)-\sum_{m=0}^{M-1}\left(\vect{y}_{k',m}-{g}_{k',m} \vect{s}_{k'} r_{k'}e^{\jmath\phi_{k'}}\right)^H\nonumber\\
&\mat{C}^{-1}
\left(\vect{y}_{k',m}-{g}_{k',m} \vect{s}_{k'} r_{k'}e^{\jmath\phi_{k'}}\right),
\end{align*}
where we explicitly express the dependence in $(r_{k'},\phi_{k'})$ while the other $(r_{k},\phi_{k}),k\neq k'$ do not appear since they are considered constant. Note that the matrix $\mat{C}$, defined in (\ref{eq:covariance_matrix_C}), does not depend on $\phi_{k'}$ but only $r_{k'}$. In the extreme case of no prior \gls{csi}, \textit{i.e.}, $g_{k',m}=0$ $\forall m$, the dependence of $f(r_{k'},\phi_{k'})$ in $\phi_{k'}$ disappears and there is an underdetermination and no estimate of the phase offset can be obtained. In other cases, we can find that, after some manipulations,
\begin{align}
	%\frac{df}{d\phi_{k'}}=0\leftrightarrow
 \hat{\phi}_{k'}&=\angle  \vect{s}_{k'}^H \mat{C}^{-1}      \sum_{m=0}^{M-1}{g}_{k',m}^*  \vect{y}_{k',m}. \label{eq:phase_update}
\end{align}
This result has an intuitive understanding: the optimal phase $\phi_k'$ tends to align the partial \gls{csi} with the observations due to device $k'$. 

\subsubsection{Removing the phase dependence}

Inserting this optimal value in the objective function $f(r_{k'},\phi_{k'})$ makes the dependence in $\phi_{k'}$ vanish and gives
\begin{align}
f(r_{k'})
&=-M\ln\left(\left|\mat{C}\right|\right)-\sum_{m=0}^{M-1}\vect{y}_{k',m}^H
\mat{C}^{-1}
\vect{y}_{k',m}\nonumber\\
&-r_{k'}^2
\vect{s}_{k'}^H\mat{C}^{-1}\vect{s}_{k'} \sum_{m=0}^{M-1}|g_{k',m}|^2\nonumber\\
&+2\left|\sum_{m=0}^{M-1}\vect{y}_{k',m}^H
\mat{C}^{-1} \vect{s}_{k'} {g}_{k',m}\right|r_{k'}. \label{eq:f_r_k_prime}
\end{align}

\subsubsection{Amplitude optimization}

To alleviate the dependence on $r_{k'}$ in (\ref{eq:f_r_k_prime}), 
% In the expression of $f(r_{k'})$, a complex modulus of an expression that depends on $r_{k'}$ has appeared, which complicates differentiation. To alleviate this and make the dependence in $r_{k'}$ more clear, 
let us define
\begin{align}
	\mat{C}_{-k'}&=\mat{C}-\lambda_{k'}^2|\gamma_{k'}|^2 \vect{s}_{k'}\vect{s}_{k'}^H\label{eq:C_minus_k_prime}\\
	&=\sum_{k\setminus k'}\lambda_k^2|\gamma_k|^2 \vect{s}_k\vect{s}_k^H +\sigma^2\mat{I}_T, \nonumber
\end{align}
which does not depend on $r_{k'}$ and is full rank, thus invertible. Applying the Sherman-Morrison formulas
\begin{align}
	\left(\mat{A} + \vect{u}\vect{v}^\textsf{T}\right)^{-1} &= \mat{A}^{-1} - \frac{\mat{A}^{-1}\vect{u}\vect{v}^\textsf{T}\mat{A}^{-1}}{1 + \vect{v}^\textsf{T}\mat{A}^{-1}\vect{u}}\nonumber\\
	\left(\mat{A} + \vect{u}\vect{v}^\textsf{T}\right)^{-1}\vect{u} %&= \mat{A}^{-1}\vect{u} - \frac{\mat{A}^{-1}\vect{u}\vect{v}^\textsf{T}\mat{A}^{-1}\vect{u}}{1 + \vect{v}^\textsf{T}\mat{A}^{-1}\vect{u}}
	&= \frac{\mat{A}^{-1}\vect{u}}{1 + \vect{v}^\textsf{T}\mat{A}^{-1}\vect{u}} \label{eq:Sherman_Morrison_formula}
\end{align}	
to $\mat{C}^{-1}$ and $\mat{C}^{-1}\vect{s}_{k'}$ gives
\begin{align}
	\mat{C}^{-1}& =\mat{C}_{-k'}^{-1}-\frac{\mat{C}_{-k'}^{-1}\vect{s}_{k'}\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}r_{k'}^2\lambda_{k'}^2}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}\label{eq:C_inverse_Sherman_Morrison_formula}\\
% 	\mat{C}^{-1}\vect{s}_{k'}r_{k'}\lambda_{k'}&=\frac{\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}\lambda_{k'}}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}\\
	\mat{C}^{-1}\vect{s}_{k'}&=\frac{\mat{C}_{-k'}^{-1}\vect{s}_{k'}}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2} \label{eq:C_inverse_s_Sherman_Morrison_formula}
\end{align}
% Inserting these expression in (\ref{eq:f_r_k_prime}), the objective function becomes
% \begin{align*}
% f(r_{k'})%&=-M\ln\left(\left|\mat{C}\right|\right)-MT\ln(\pi)\\
% % &-\sum_{m=0}^{M-1}\vect{y}_{k',m}^H
% % \mat{C}^{-1}
% % \vect{y}_{k',m}-r_{k'}^2
% % \vect{s}_{k'}^H\mat{C}^{-1}\vect{s}_{k'} \sum_{m=0}^{M-1}|g_{k',m}|^2+2\left|  \frac{\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}{g}_{k',m}}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2} \right|r_{k'}\\
% &=-M\ln\left(\left|\mat{C}\right|\right)-\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}^{-1}\vect{y}_{k',m}\\
% &-r_{k'}^2 \vect{s}_{k'}^H\mat{C}^{-1}\vect{s}_{k'} \sum_{m=0}^{M-1}|g_{k',m}|^2+2  \frac{\left|\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}{g}_{k',m}\right|}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}r_{k'}
% \end{align*}
% Good news, the differenciability problem seems to be solved. Now we apply the Sherman-Morrison formula on each inverse to put in evidence the dependence in $r_{k'}$. 
We insert these expressions in (\ref{eq:f_r_k_prime}) and we omit terms that do not depend on $r_{k'}$, which will vanish after taking the derivative. This gives
\begin{align}
\tilde{f}(r_{k'})%&=-M\ln\left(\left|\mat{C}\right|\right)+\sum_{m=0}^{M-1}\vect{y}_{k',m}^H
% \frac{\mat{C}_{-k'}^{-1}\vect{s}_{k'}\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}r_{k'}^2\lambda_{k'}^2}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}
% \vect{y}_{k',m}\\
% &-r_{k'}^2
% \frac{\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2} \sum_{m=0}^{M-1}|g_{k',m}|^2+2  \frac{\left|\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}{g}_{k',m}\right|}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}r_{k'}\\
%&=-M\ln\left(\left|\mat{C}\right|\right)+\sum_{m=0}^{M-1}
% \frac{|\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}|^2\lambda_{k'}^2r_{k'}^2}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}\\
%&-r_{k'}^2\frac{\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2} \sum_{m=0}^{M-1}|g_{k',m}|^2+2  \frac{\left|\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}{g}_{k',m}\right|}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}r_{k'}\\
&=-M\ln\left(\left|\mat{C}\right|\right)+\frac{\alpha r_{k'}^2+\beta r_{k'}}{1+\delta r_{k'}^2}, \label{eq:f_tilde}
\end{align}
where we defined the constants (independent of $r_{k'}$) $\alpha$, $\beta$ and $\delta$, as
\begin{align}
	\alpha&=\sum_{m=0}^{M-1}
	{|\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}|^2\lambda_{k'}^2}-
	{\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}} \sum_{m=0}^{M-1}|g_{k',m}|^2\nonumber\\
	\beta&=2  \left|\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}{g}_{k',m}\right|\nonumber\\
	\delta&=\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}\lambda_{k'}^2. \label{eq:alpha_beta_gamma}
\end{align}
One can note that $\tilde{f}(r_{k'})$ in (\ref{eq:f_tilde}) can now be differentiated with respect to $r_{k'}$, using the differential rule $\partial (\log |\mat{A}|)=\tr[\mat{A}^{-1} \partial \mat{A}]$. Setting the derivative to zero gives, noting that the denominator is always strictly positive,
\begin{align}
	\frac{d\tilde{f}}{dr_{k'}}&=0\nonumber\\
	\leftrightarrow 0&=-r_{k'}^32M\delta^2-r_{k'}^2\beta\delta+r_{k'}(-2M\delta+2\alpha)+\beta, \label{eq:update_partial_CSI}
\end{align}
which is a polynomial of degree~3 in $r_{k'}$. There are closed-form solutions for the roots of such polynomials. Following \textit{Descarte's rule of signs}, (\ref{eq:update_partial_CSI}) has only one real and positive root, as required, in case the terms are non-zero. Below we discuss the special cases when the terms are not non-zero, i.e., when there is no or complete \gls{csi} knowledge.


%One should still check for the best solutions among them, restricted to be positive and real.\footnote{even though we could not prove it analytically, in all our simulations only one such root was found, solving this root selection problem.}

The algorithm is summarized in the pseudocode \textbf{Algorithm~\ref{alg:cap}}. At each iteration, the constants $\alpha$, $\beta$ and $\delta$ can be easily re-evaluated based on~(\ref{eq:alpha_beta_gamma}). One can note that they require the matrix inversion $\mat{C}_{-k'}^{-1}$. To avoid re-computing a full inverse at each iteration, one can rely on the Sherman-Morrison formula and on the current knowledge of $\mat{C}^{-1}$, which is updated at the end of each iteration by inserting the obtained value of $r_{k'}$ in~(\ref{eq:C_inverse_Sherman_Morrison_formula}). Using~(\ref{eq:C_minus_k_prime}) and~(\ref{eq:Sherman_Morrison_formula}), we find
% \begin{align}
%     \mat{C}_{-k'}^{-1}\vect{s}_{k'}&=\left(\mat{C}-\lambda_{k'}^2|\gamma_{k'}|^2 \vect{s}_{k'}\vect{s}_{k'}^H\right)^{-1}\vect{s}_{k'} \nonumber\\
% 	&= \frac{\mat{C}^{-1}\vect{s}_{k'}}{1 -  \lambda_{k'}^2|\gamma_{k'}|^2 \vect{s}_{k'}^H \mat{C}^{-1}\vect{s}_{k'}}. \label{eq:C_minus_k_prime_Sherman_Morrison}
% \end{align}
\begin{align}
    \mat{C}_{-k'}^{-1}&=\left(\mat{C}-\lambda_{k'}^2|\gamma_{k'}|^2 \vect{s}_{k'}\vect{s}_{k'}^H\right)^{-1}\nonumber\\
	&= \mat{C}^{-1}+\frac{\lambda_{k'}^2|\gamma_{k'}|^2 \mat{C}^{-1}\vect{s}_{k'}\vect{s}_{k'}^H\mat{C}^{-1} }{1 -  \lambda_{k'}^2|\gamma_{k'}|^2 \vect{s}_{k'}^H \mat{C}^{-1}\vect{s}_{k'}}. \label{eq:C_minus_k_prime_Sherman_Morrison}
\end{align}
Moreover, computations can be optimized as several quantities appear multiple times and can be computed only once. We now investigate two particular cases, to gain further insights.

\begin{algorithm}
\caption{Iterative maximum likelihood device activity detector}\label{alg:cap}
\small 
\begin{algorithmic}
\Require $\sigma^2,\lambda_k,\vect{y}_m, g_{k,m}, \hat{\vect{\gamma}}_{\mathrm{init}} \ \forall k,m$
\State $k' \gets 0$
\State $\hat{\vect{\gamma}} \gets \hat{\vect{\gamma}}_{\mathrm{init}}$
\State $\mat{C}^{-1} \gets \left(\sum_{k=0}^{K-1}\lambda_k^2|\hat{\gamma}_k|^2 \vect{s}_k\vect{s}_k^H +\sigma^2\mat{I}_T\right)^{-1}$
\While{Not converged}

    Compute $\vect{y}_{k',m}$, $\mat{C}_{-k'}^{-1}$, $\alpha$, $\beta$ and $\delta$ based on (\ref{eq:y_m_k_prime}), (\ref{eq:C_minus_k_prime_Sherman_Morrison}) and (\ref{eq:alpha_beta_gamma})

    \State $\hat{r}_{k'} \gets \arg \max \tilde{f}(r_{k'})$ \Comment{Update amplitude based on (\ref{eq:update_partial_CSI}), (\ref{eq:update_no_CSI}) or (\ref{eq:update_prior_CSI})}
    \State $\hat{\phi}_{k'} \gets \angle  \vect{s}_{k'}^H \mat{C}^{-1}      \sum_{m=0}^{M-1} {g}_{k',m}^*  \vect{y}_{k',m}$ \Comment{Update phase}
    \State $\hat{\gamma}_{k'} \gets \hat{r}_{k'}e^{\jmath \hat{\phi}_{k'}}$
    \State $\mat{C}^{-1} \gets \mat{C}_{-k'}^{-1}-\frac{\mat{C}_{-k'}^{-1}\vect{s}_{k'}\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}r_{k'}^2\lambda_{k'}^2}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}$
    \State $k' \gets k'+1 \mod K$
\EndWhile
\end{algorithmic}
\end{algorithm}



\paragraph{Particular case: device with no \gls{csi}}

Now consider that, for a given $k'$, ${g}_{k',m}={0}\  \forall m$. This could be because this device is new or moving a lot such that its \gls{csi} is outdated. Only, its parameter $\lambda_{k'}$ is known, which is equal to the large-scale fading coefficient $\sqrt{\beta_{k'}}$. At iteration of user $k'$, evaluating (\ref{eq:alpha_beta_gamma}) for ${g}_{k',m}={0}\  \forall m$ implies that $\beta=0$. Hence, (\ref{eq:update_partial_CSI}) simplifies to
\begin{align*}
	0=2r_{k'}(-r_{k'}^2M\delta^2-M\delta+\alpha),
\end{align*}
which has a trivial solution in $r_{k'}=0$. One of the other roots is always negative. Keeping only the positive one, we find the amplitude update
\begin{align}
\hat{r}_{k'}=\sqrt{\frac{\alpha-M\delta}{M\delta^2}}. \label{eq:update_no_CSI}
\end{align}
If this root is imaginary, we set $\hat{r}_{k'}$ to zero. As discussed before introducing the phase update equation~(\ref{eq:phase_update}), in the case of no prior \gls{csi}, the phase ambiguity cannot be resolved. This particular case gives an update relatively similar to the maximum likelihood estimator derived in~\cite[(23)]{FenglerTIT}, where their \gls{ml} expression estimates the error, while ours estimates directly the coefficient $\hat{r}_{k'}$, given the same estimate of $\gamma_{k'}$ at each iteration.

%\TODO{The reader may wonder, are they identical, and if not, wherein lies the difference and why?}

% A similar, simplified, iterative algorithm can be used to maximize the likelihood. At iteration of user $k'$, the function to be maximized $f(r_{k'},\phi_{k'})$ simplifies to
% \begin{align*}
% f(r_{k'},\phi_{k'})&=-M\ln\left(\left|\mat{C}\right|\right)-MT\ln(\pi)-\sum_{m=0}^{M-1}\vect{y}_{k',m}^H\mat{C}^{-1} \vect{y}_{k',m},
% \end{align*}
% which does not depend on $\phi_{k'}$. Hence, the phase cannot be resolved. Using Sherman-Morrison formula (\ref{eq:C_inverse_Sherman_Morrison_formula}) and keeping only the terms that depend on $r_{k'}$ gives
% \begin{align*}
% \tilde{f}(r_{k'})&=-M\ln\left(\left|\mat{C}\right|\right)+\sum_{m=0}^{M-1}
% \frac{|\vect{y}_{k',m}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}|^2\lambda_{k'}^2r_{k'}^2}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}r_{k'}^2\lambda_{k'}^2}\\
% &=-M\ln\left(\left|\mat{C}\right|\right)+\frac{\alpha r_{k'}^2}{1+\delta r_{k'}^2},
% \end{align*}
% where we used previous definitions. In this particular case, only the magnitude square $r_{k'}^2$ appears so that we can optimize (given their one-to-one relationship for $r_{k'}\in \mathbb{R}^+$) with respect to $p_{k'}=r_{k'}^2$.
% \begin{align*}
% \tilde{f}(p_{k'})&=-M\ln\left(\left|\mat{C}\right|\right)+\frac{\alpha p_{k'}}{1+\delta p_{k'}} 
% \end{align*}
% Taking the derivative and applying Sherman-Morrison formula (\ref{eq:C_inverse_s_Sherman_Morrison_formula}) gives
% \begin{align*}
% \frac{d\tilde{f}}{dp_{k'}}&=-M\lambda_k^2 \vect{s}_k^H\mat{C}^{-1} \vect{s}_k +\frac{\alpha(1+\delta p_{k'})-\alpha p_{k'}\delta }{\left(1+\delta p_{k'}\right)^2}\\
% % &=-M\lambda_k^2 \frac{\vect{s}_k^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}}{1+\vect{s}_{k'}^H\mat{C}_{-k'}^{-1}\vect{s}_{k'}p_{k'}\lambda_{k'}^2} +\frac{\alpha}{\left(1+\delta p_{k'}\right)^2}\\
% &=- M\frac{\delta }{1+\delta p_{k'}} +\frac{\alpha}{\left(1+\delta p_{k'}\right)^2}.
% \end{align*}
% Setting the derivative to zero gives (noting that the denominator is always strictly positive)
% \begin{align}
% \frac{d\tilde{f}}{dp_{k'}}&=0%\\
% % 0&=-M \delta (1+\delta p_{k'}) +\alpha\\
% % 0&=-M\delta^2 p_{k'} -M\delta+\alpha\\
% \leftrightarrow \hat{r}_{k'}=\sqrt{\frac{\alpha-M\delta}{M\delta^2}}, \label{eq:update_no_CSI}
% \end{align}
% which is much simpler to compute.



\paragraph{Particular case: device with complete prior \gls{csi}}

Now, consider that, for a given $k'$, $\lambda_{k'}={0}$, so that the \gls{csi} is perfectly known. Only the phase shift and the transmit power are unknown. At iteration of user $k'$, evaluating (\ref{eq:alpha_beta_gamma}) for $\lambda_{k'}={0}$ implies that $\delta=0$. Hence, (\ref{eq:update_partial_CSI}) simplifies to a linear equation $0=r_{k'}2\alpha+\beta$, which gives the following amplitude update
\begin{align}
\hat{r}_{k'}&=\frac{-\beta}{2\alpha}=\frac{| \vect{s}_{k'}^H
	\mat{C}^{-1} 
	\sum_{m=0}^{M-1}{g}_{k',m}^*\vect{y}_{k',m}|}{\vect{s}_{k'}^H
	\mat{C}^{-1} 
	\vect{s}_{k'} \sum_{m'}|{g}_{k',m'}|^2   },\label{eq:update_prior_CSI}
\end{align}
while the phase is updated according to (\ref{eq:phase_update}).

% \TODO{this is similar to our conference paper, but for a single device. Not sure this case really happens in practice since there is always a bit or noise/mobility on channel estimate. Even if correlation is very high like 0.99, not perfect...}


% At iteration of user $k'$, the objective function to be maximized is
% \begin{align*}
% f(\gamma_{k'})&=-M\ln\left(\left|\mat{C}\right|\right)-\sum_{m=0}^{M-1}\left(\vect{y}_{k',m}-{g}_{k',m} \vect{s}_{k'} \gamma_{k'}\right)^H
% \mat{C}^{-1}
% \left(\vect{y}_{k',m}-{g}_{k',m} \vect{s}_{k'} \gamma_{k'}\right),
% \end{align*}
% where we kept the dependence on the complex variable $\gamma_{k'}$ on purpose. Indeed, one can check that this function is concave in $\gamma_{k'}$. Indeed, $\mat{C}$, defined in (\ref{eq:covariance_matrix_C}), does not depend on $\gamma_{k'}$ given that $\lambda_{k'}=0$. Hence, $f(\gamma_{k'})$ is a quadratic function in $\gamma_{k'}$. Taking the Wirtinger derivative of $f(\gamma_{k'})$ with respect to $\gamma_{k'}^*$ and setting it to zero gives
% \begin{align}
% \frac{df}{d\gamma_{k'}^*}&=0%\\
% % 0&=\sum_{m=0}^{M-1}{g}_{k',m}^* \vect{s}_{k'}^H
% % \mat{C}^{-1} 
% % \left(\vect{y}_{k',m}-{g}_{k',m} \vect{s}_{k'} \gamma_{k'}\right)\\
% \leftrightarrow \hat{\gamma}_{k'}=\frac{ \vect{s}_{k'}^H
% 	\mat{C}^{-1} 
% 	\sum_{m=0}^{M-1}{g}_{k',m}^*\vect{y}_{k',m}}{\vect{s}_{k'}^H
% 	\mat{C}^{-1} 
% 	\vect{s}_{k'} \sum_{m'}|{g}_{k',m'}|^2   }. \label{eq:update_prior_CSI}
% \end{align}

\subsubsection{Initialization}

To start the iterative algorithm, we consider different choices to initialize $\hat{\vect{\gamma}}_{\mathrm{init}}$. A simple choice is to initialize to zero, \textit{i.e.}, $\hat{\vect{\gamma}}_{\mathrm{init}}^{0}=\vect{0}$. Another choice is to initialize solely based on the available prior \gls{csi}, considering that $\lambda_k \approx 0,\ \forall k$. The estimator is similar to \cite{callebaut2021grant}, except that, here, prior \gls{csi} is used instead of complete \gls{csi}. 

If $\lambda_k \approx 0,\ \forall k$, the covariance matrix $\mat{C}$, defined in (\ref{eq:covariance_matrix_C}), simplifies to $\mat{C}=\sigma^{-2}\mat{I}_T$, which is independent of $\gamma_k$. Hence, many terms of the log-likelihood in (\ref{eq:log_likelihood}) become independent of $\vect{\gamma}$. Maximizing (\ref{eq:log_likelihood}) becomes equivalent to the following minimization
\begin{align*}
    \max_{\vect{\gamma}} \log p(\vect{y}|\vect{\gamma})&=\min_{\vect{\gamma}}\sum_{m=0}^{M-1}\left\|\vect{y}_{m}-\sum_{k=0}^{K-1} {g}_{k,m} \vect{s}_{k} \gamma_k\right\|^2\\
    &=\min_{\vect{\gamma}}\left\|\vect{y}-\mat{\Gamma} \vect{\gamma}\right\|^2,
\end{align*}
where we defined the vector and matrix notations
\begin{align*}
    &\vect{y}=\begin{pmatrix}
    \vect{y}_{0}\\
    \vdots\\
    \vect{y}_{M-1}
    \end{pmatrix},\ \mat{\Gamma}= \begin{pmatrix}
    \mat{\Gamma}_{0}\\
    \vdots\\
    \vect{\Gamma}_{M-1}
    \end{pmatrix},\\
    &\mat{\Gamma}_m=\begin{pmatrix}
    \vect{s}_{0} & \hdots & \vect{s}_{K-1}
    \end{pmatrix} \diag{ (g_{0,m}, \hdots g_{{K-1},m})}.
\end{align*}
This minimization problem is a quadratic function of $\vect{\gamma}$, which is a least squares problem. The estimate has the following closed-form expression
\begin{align}
    \hat{\vect{\gamma}}_{\mathrm{init}}^{\mathrm{ZF}}&= \left(\mat{\Gamma}^H \mat{\Gamma}\right)^{-1} \mat{\Gamma}^H \vect{y}.
    \label{eq:zf}
\end{align}
This last estimator can be seen as a \gls{zf} estimator, which requires a matrix inversion. To avoid ill-conditioning, a first necessary condition is that $K\leq M T$. This condition is not sufficient as the channel and preamble of two devices could be correlated, especially when $K$ is on the order of $MT$. Moreover, if no prior information is available for a given user $k'$, \textit{i.e.}, $g_{k',m}=0,\ \forall m$, the inverse will also be ill-conditioned. This implies that the $k'$-th column of $\mat{\Gamma}$ becomes null and thus $\mat{\Gamma}$ is rank deficient. Moreover, the prior \gls{csi} might be noisy, leading to unstable results.

To make initialization more robust, we can use an \gls{lmmse} criterion. To do this, some prior knowledge must be assumed on the statistics of $\vect{\gamma}$, more specifically, its first and second order moments. We here make the following assumptions: i) the activity of each device is independent of one another, ii) the average activity and average transmit power of each device is known and iii) no prior information is known on the phase offset so that $\phi_k$ is considered uniformly distributed between 0 and $2\pi$. Under these assumptions, we have $\mathbb{E}(\vect{\gamma})=\vect{0}$ and $\mat{D}=\mathbb{E}(\vect{\gamma}\vect{\gamma}^H)=\diag\left(\mathbb{E}(a_0)\mathbb{E}(\rho_0),...,\mathbb{E}(a_{K-1})\mathbb{E}(\rho_{K-1})\right)$. Hence, for the linear observation model $\vect{y}=\mat{\Gamma} \vect{\gamma} + \vect{w}$, still considering that $\lambda_k \approx 0,\ \forall k$, the \gls{lmmse} estimator of $\vect{\gamma}$ is then given by \cite{kay1993fundamentals}
\begin{align}
\hat{\vect{\gamma}}_{\mathrm{init}}^{\mathrm{LMMSE}}&= \left(\mat{\Gamma}^H \mat{\Gamma} + \sigma^2 \mat{D}^{-1} \right)^{-1} \mat{\Gamma}^H  \vect{y}.
    \label{eq:lmmse}
\end{align}
Note that the matrix to be inverted is always well-conditioned. Finally, a \gls{mf} estimator could be used to avoid the need for matrix inversion.
\begin{align}
    \hat{\vect{\gamma}}_{\mathrm{init}}^{\mathrm{MF}}&= \left(\diag(\mat{\Gamma}^H \mat{\Gamma}) + \sigma^2 \mat{D}^{-1} \right)^{-1} \mat{\Gamma}^H  \vect{y}.
    \label{eq:mf}
\end{align}

\subsection{Activity Detection}

A non-negative activity threshold $\gamma_{\text{th},k}$ is applied for each device $k$. A device is considered active if $\abs{\hat{\gamma}_k} \geq \gamma_{th,k}$. 
The real-valued threshold is defined as,
\begin{equation}\label{eq:threshold}
    \gamma_{\text{th}, k} = v \sqrt{\text{SNR}_k}^{-1},
\end{equation}
where $v$ is chosen to have a desired probability of false alarm and miss detection performance and with $\text{SNR}_k = M\beta_k / \sigma^2  = \mathbb{E}(\norm{\vect{h}_k}^2) / \sigma^2  =(\norm{\vect{g}_k}^2+M\lambda_k^2) / \sigma^2$. 

Miss detection happens when a device was undetected, while it was actually transmitting. Equivalently, a false alarm occurs if a device is considered active by the algorithm but was not. We define the probability of miss detection as the average ratio of undetected devices to the number of active devices
\begin{equation*}
    \prob_{\mathrm{md}} = 1 - \expt{
            \dfrac{
                \abs{\mathcal{K}_a \cap \hat{\mathcal{K}}_a }
            }{
                \abs{\mathcal{K}_a}
            }
        },
\end{equation*}
where $\mathcal{K}_a$ is the set of active devices and $\hat{\mathcal{K}}_a = \{k | \hat{a}_k=1, \forall \in [1,K]\}$ denotes the estimated set of active devices.
Note that on average $\abs{\mathcal{K}_a}=K_a$.
Similarly, the probability of false alarm is the ratio of inactive devices considered active to the number of inactive devices and is given by
\begin{equation*}
    \prob_{\mathrm{fa}} = \expt{
            \dfrac{
                \abs{\hat{\mathcal{K}}_a \setminus  \mathcal{K}_a}
            }{
                K - \abs{\mathcal{K}_a}
            }
    }.
\end{equation*}

A trade-off can be made between the two probabilities by varying $v$ in~(\ref{eq:threshold}). A lower $v$ yields a lower activity threshold, resulting in more devices considered active. This in turn lowers the probability of miss detection, while increasing the probability of generating a false alarm. In the simulations, the parameter $v$ is swept across the range $[-40, 40]$\,\si{\deci\bel}. 

%To conveniently study the impact of different parameters, the metric \textit{error probability} is introduced $\prob_{e}=\prob_{\text{md}}=\prob_{\text{fa}}$.\footnote{\update{This metric is an approximation, where we numerically find $\prob_{\text{md}} \approx \prob_{\text{fa}}$ by finding the threshold where $\argmin{| \prob_{\text{md}} - \prob_{\text{fa}} | }$.}}

==> rev/before-pruning-for-wcnc/Section/Experimental_Results.tex <==
\section{Numerical Assessment}
\label{section:experimental_results}
\begin{table}[htbp]
    \centering
    \renewcommand*{\arraystretch}{1.2}
    \caption{Simulation parameter set with default values.}
    \label{tab:initial-access-setup}
    \centering
    \footnotesize
      \begin{threeparttable}
    \begin{tabular}{@{}lll@{}}
    \toprule
    Parameter &  Symbol & Default value\\ \midrule
    
    Number of devices & $K$ & \num{500}\\
    %Number of \glspl{ap} & $N$ & -\\
    Number of total \gls{bs} antennas & $M$ & 64\\
    \Acrlong{snr} &  \acrshort{snr}  & \SI{20}{\deci\bel}\\
    Device activity probability & $\epsilon_a$ & \num{0.1}\\
    % Transmit power of the device & $\rho$ & \SI{1}{\milli\watt}\\
    % Bandwidth & $B$ & \SI{125}{\kilo\hertz}\\
    % Thermal noise &$\sigma^2$ & \SI{-122.88}{\dBm} \\
    Pilot sequence & $s_k$ & $\cn{0}{1}$\\
    Pilot length &$\tau_p$  & \num{10} symbols\\
    Phase offset & $\phi_k$ &$\sim\mathcal{U}_{[0, 2\pi]}$\\
    Number of simulations & $N_\text{sim}$ & $>$\num{10000}\\
    Number of algorithm iterations & $N_\text{iter}$ & $K \cdot 4$\\
    Initialization vector & $\hat{\vect{\gamma}_\text{init}}$ & $\hat{\vect{\gamma}}_{\mathrm{init}}^{\mathrm{LMMSE}}$ (\ref{eq:lmmse})\\
    Unknown part of the \gls{csi} & $\lambda$ & \num{0.3}\\
    \bottomrule
    \end{tabular}
    \end{threeparttable}
    \end{table}

The default simulation configurations are summarized in Table~\ref{tab:initial-access-setup}. 
The device activity profile is generated randomly and independently for each device with a probability $\epsilon_a=0.1$, meaning that on average $\epsilon_a K = 50$ devices are active simultaneously. Or equivalently, the devices have an average duty cycle of 10\%, which is high for typical \gls{iot} applications~\cite{s21030913}.
The channel between the \gls{bs} and device $k$ is modelled as in (\ref{eq:prior_CSI_channel_model}).
The pilot sequence is randomly generated from a complex Gaussian distribution $s_k \cn{0}{1}$, and is assumed to be known by the \gls{bs}. Each device uses a pilot sequence of \num{10}~symbols. A random phase offset $\phi_k \sim\mathcal{U}_{[0, 2\pi]}$ is generated to simulate a \acrlong{cfo} (considered time-invariant over the preamble duration). The source code for all simulations can be accessed online\footnote{\url{https://github.com/wavecore-research/grant-free-random-access-partial-csi}}.


\subsection{Convergence of different initialization vectors}

The convergence of different initializations is evaluated with respect to the genie-aided approach. In the genie-aided case, the algorithm is initialized with the real activity indicators, i.e., $\vect{\gamma}$. The convergence is assessed via the likelihood (\ref{eq:log_likelihood}) and the \gls{mse}. The former should monotonically increase with each iteration, while the \gls{mse} can vary as it can not directly be minimized. 
The performance of the different initialization vectors for $\hat{\vect{\gamma}}_{\text{init}}$ are depicted in Figure~\ref{fig:convergence}. The bottom figures zoom in on a smaller region to distinguish the performance of the initialization vectors when converging closer to the genie-aided case.  
While all initialization methods approximate the genie-aided case, the initialization vector has a non-negligible impact on the performance of the algorithm. An intuitive approach is to initialize with $\vect{0}$ because the activity probability is low and hence, on average, \SI{90}{\percent} of the devices are expected to be inactive. As illustrated in Figure~\ref{fig:convergence}, $\hat{\vect{\gamma}}_{\text{init}}=\vect{0}$ requires considerably more iterations to approach the other initialization methods.

\begin{figure*}[h]
    \begin{center}
         \begin{subfigure}[b]{0.8\columnwidth}
            \input{Fig/convergence_llh.tex}
        \end{subfigure}\hspace{0.9cm}
         \begin{subfigure}[b]{0.8\columnwidth}
            \input{Fig/convergence_mse.tex}
        \end{subfigure}
    \end{center}\vspace{-1cm}
    \begin{center}
        \begin{subfigure}[b]{0.8\columnwidth}
            \input{Fig/convergence_llh_zoomed.tex}
        \end{subfigure}\hspace{0.9cm}
        \begin{subfigure}[b]{0.8\columnwidth}
            \input{Fig/convergence_mse_zoomed.tex}
        \end{subfigure}
    \end{center}\vspace{-0.5cm}
    \caption{The log-likelihood (\ref{eq:log_likelihood}) and \gls{mse} of the estimated activity indicators for different initialization vectors. While with all initialization vectors the genie-aided case is approximated, different number of iterations are required.}\label{fig:convergence}
\end{figure*}



\subsection{Impact of the quality of prior CSI}

Figure~\ref{fig:lambda_prob_gain} illustrates the performance of the detector algorithms for different correlations between the actual channel and the known \gls{csi}, i.e., $\lambda$. 
With increased $\lambda$, and thus decreased channel knowledge, both the \gls{lmmse} estimator and the proposed algorithm have an increased probability of miss detection. The figure also demonstrates the gain of the proposed algorithm with respect to the \gls{lmmse} estimator. The algorithm outperforms the \gls{lmmse} estimator for all $\lambda$ and is most effective when the prior \gls{csi} has a strong correlation with the actual channel, and diminishes with decreased channel knowledge.



\begin{figure}[h]
    \centering
        %\input{Fig/lambda_prob_gain_100}
        \input{Fig/lambda_prob}
    \caption{\small Performance of the proposed algorithm (\ref{algo}) versus the \Gls{lmmse} estimator (\ref{rzf}) for different values of channel knowledge. The probability of miss detection is shown for different values of $\prob_{\mathrm{fa}}$ (\SI{10}{\percent}, \SI{1}{\percent}, \SI{0.1}{\percent}).}\label{fig:lambda_prob_gain}
\end{figure}

\subsection{Impact of the \acrlong{snr}}

Figure~\ref{fig:fa_md_snrs} shows the false alarm and miss detection probability of the \gls{lmmse} estimator and the iterative maximum likelihood device activity detector for different device \glspl{snr}. The full \gls{csi} case is included as a baseline for comparison, where the full \gls{csi} is known instead of only a portion ($\lambda$). Fig.~\ref{fig:fa_md_snrs} demonstrates the large performance gain of the proposed algorithm with respect to the \gls{lmmse} estimator. The graph demonstrates that the iterative algorithm lowers the probability of miss detection by a factor of 21 for the same probability of false alarm.\footnote{Notably, the \gls{lmmse} estimator does not employ an iterative approach. Therefore, our proposed algorithm will be compared in future work with other iterative approaches.} The performance is only marginally increased for very low \glspl{snr} (below zero). 


\begin{figure}[h]
    \centering


        \input{Fig/fa_md_snrs.tex}
    \caption{\small The probability of false alarm and miss detection for different device \glspl{snr} for the \gls{lmmse} estimator when having full \gls{csi} ({\color{black} \ref{full}}) and partial \gls{csi} (\ref{rzf}), and the proposed iterative algorithm with partial \gls{csi} (\ref{algo}). No miss detection or false alarm occurred in the full \gls{csi} case for \gls{snr} values of \SI{-6.67}{\deci\bel} and \SI{20}{\deci\bel}.}\label{fig:fa_md_snrs}
\end{figure}

% \subsection{Achievable Rate}
% \begin{align}
%     R_k = \expt{\log_2(1+\text{SINR}_k)}
% \end{align}

% \begin{align}
%     R_{\text{sum}} = \sum\nolimits_{k \in \mathcal{K}_a} R_k
% \end{align}
% This figure of merits penalties when non-active users are included in the detector matrix, and also when active users were considered inactive. \gilles{Notably, the sum-rate could be higher even when not all active users are considered with respect to when all active users are included.}


==> rev/before-pruning-for-wcnc/Section/Introduction.tex <==
\section{Introduction}
\Gls{mmtc} is envisioned to enable low-power connectivity to a very large number of devices and open up new applications. While it has been put forward as a key building block in 5G and beyond, it has so far received less attention than \gls{embb} and \gls{urllc}.
% While current endeavors in 5G and beyond systems have focused on providing high spectral efficiency (\gls{embb}) and low-latency (\gls{urllc}), \gls{mmtc} has received less attention.
The challenge in \gls{mmtc}, and in general \gls{iot} systems, resides in the low-power operation, sporadic nature of the traffic and a large amount of uncoordinated devices. As these devices are often battery-powered, they are constrained in the signalling overhead they can handle~\cite{s21030913}. Furthermore, they are often deployed in remote areas, where network coverage is low or non-existent~\cite{s21030913,9443344}. To address this, novel protocols need to be designed tailored to the low-power, sporadic and massive nature of \gls{mmtc} traffic. One promising direction, and the focus of this work, is the use of massive MIMO, where a large number of antennas is present at the base station.

Two multiple access approaches can be taken, grant-based and grant-free random access. The former requires the devices to obtain a grant from the network, where after it can use  a collision-free radio resource to transmit its data. The disadvantage of this approach for \gls{iot} and \gls{mmtc} is that devices need to compete for grants, requiring, e.g., dedicated preambles or a lot of signalling for collision resolution. Due to the number of competing devices such schemes are not practical and scalable.  

Therefore, grant-free approaches are advocated over grant-based solutions~\cite{8454392, 8456557, 9049039}. In grant-free random access, devices do not contend for a grant, but just access the network when required. Often these devices are unaware of the other devices in the system and operate in an uncoordinated fashion, which is called unsourced grant-free random access~\cite{9049039}. Different approaches have been studied to detect the active devices in massive MIMO systems. Detecting active devices is facilitated when each device uses a unique and orthogonal preamble sequence. This entails that each preamble should have the same length as the number of devices to have no collisions, which is unpractical. Therefore a number of studies have considered a pool of orthogonal pilots~\cite{9091017} or the use of non-orthogonal pilots. Both of these strategies have been elaborated in~\cite{8454392}, where they formulate the device-activity detection problem as a compressed sensing problem, where the sparsity of the active devices at each time slot is exploited. However, compressed sensing requires the preamble length to be larger than the active devices, increasing the energy expenditure of data transfer. To combat this, in~\cite{9049039, FenglerTIT} a covariance-based method is suggested using two estimators for device activity recovery, i.e., \gls{ml} and \gls{nnls}. This work is generalized by \citeauthor{GanesanSPAWC}~\cite{GanesanSPAWC,GanesanTCOM} to the cell-free case where multiple \glspl{ap} are geographically distributed. They considered different large-scale fading coefficients per \glspl{ap}. They employed a simplification of their proposed algorithm by including only the \gls{ap} with the strongest contribution. They concluded that co-located massive MIMO is highly sensitive to low \glspl{snr}, while cell-free deployment is better suited against shadowing fading effects. 

\textbf{Contributions.} 
Inspired by these works, we propose a new algorithm exploiting the static nature of \gls{iot} devices. As demonstrated in~\cite{callebaut2021grant}, the \gls{csi} can remain almost invariant over large period of times (hours) for scenarios with low mobility. This was not yet leveraged by practical algorithms in the literature to the best of our knowledge. Given that the base station knows a part of the \gls{csi} of each device, further denoted as partial \gls{csi}, the performance of the device activity scheme can be improved. To do so, we formulate the \acrlong{ml} activity detection problem using partial \gls{csi}. The ``amount of partial CSI'' a priori known can be adapted for each user through a parameter, which can model all cases going from no prior \gls{csi} to full prior \gls{csi}. Furthermore, a phase offset can be estimated which occurs due to \gls{cfo}. Besides presenting an analytical derivation of the proposed algorithm, a numerical evaluation is performed. We validate the convergence of the iterative algorithm, study the impact of different initialization vectors for the device activity, the impact of the quality of the partial \gls{csi} and the \gls{snr} on the performance of the algorithm. We show that the presented estimator outperforms the conventional \gls{lmmse} estimator for device activity detection even for short-length preambles (10 symbols).
 


%\subsection{Problem Statement}



% \TODO{put forward ML based? not Bayesian?}
% \TODO{orient centralized or distributed?}
% \TODO{re-read latex document (draft) with key advantages, also summarized in ICC paper}

% \subsection{State-of-the-Art}
% \TODO{}


% \TODO{As a side note, the references \cite{GanesanSPAWC,GanesanTCOM} (conf and journal papers) are inspired by \cite{9049039,FenglerTIT}, which they generalize to the cell free case by considering different large scale fading coefficients per AP. Still they could not directly use the algorithm and had to simplify by considering contribution from closest AP.}


% \TODO{\cite{callebaut2021grant} full CSI}

% \cite{8454392}:
% \begin{itemize}
%     \item advocates the usage of grant-free rather than grant-based random access schemes to overcome the challenge of massive IoT access.
%     \item compressed sensing techniques (e.g., multiplemeasurement vector (MMV))
% \end{itemize}

% \cite{8456557}:
% \begin{itemize}
%     \item grant-free RA for conjugate beamforming and zero-forcing beamforming techniques
%     \item  It is confirmed that the grant-free RA with massive MIMO is an attractive RA technique with low signaling overhead that could simultaneously accommodate a number of RA users, which is multiple times the number of RA channels, with close-to-one success probability.
% \end{itemize}

% \cite{9091017}:
% \begin{itemize}
%     \item we propose a new RA scheme that inserts a base station (BS) broadcasting message after user equipments (UEs) transmitting pilots.
%     \item collision resolution, by using this broadcast message to see if collided
%     \item spectral efficiency with maximum-ratio-combing (MRC) and zero-forcing (ZF) receivers
% \end{itemize}

% \cite{8993804}:
% \begin{itemize}
%     \item performs the joint active UEs detection and uplink message decoding without channel estimation in one shot by utilizing the proposed ensemble independent component analysis (EICA) decoding algorithm
% \end{itemize}

% \cite{9049039}:
% \begin{itemize}
%     \item unsourced random access (U-RA)
%     \item Previous results, based on compressed sensing, require that $K_a \leq L$, which is a bottleneck in massive deployment scenarios such as Internet-of-Things and U-RA.
% \end{itemize}

% \cite{8770292}:
% \begin{itemize}
%     \item super preamble consisting of multiple consecutive preambles is proposed for the high success rate of grant-free RA with massive MIMO
%     \item propose a reliable UE detection algorithm to obtain the super preambles of the UEs by exploiting the quasi-orthogonality characteristic of massive MIMO
%     \item The theoretical analysis and simulation results show that turning a preamble into a super preamble consisting of two or three shorter preambles, the success rate of UE detection and channel estimation could be significantly increased using the proposed approach
% \end{itemize}




\textbf{Notations:} vectors are denoted by boldface lower case~\(\vect{x}\) and matrices by boldface capital letters~\(\mat{X}\).
The superscript \({(\cdot)}^T\) is used to denote the transpose operation. The absolute value is denoted by \(\abs{\cdot} \) for vectors and scalars, while the same notation is used to denote the determinant of a matrix.
The notation \(\expt{\cdot}\) denotes the expectation of a random variable. The set of complex numbers is denoted by the symbol \(\mathbb{C}\) and the set of strictly positive numbers by $\mathbb{R}^+$. The uniform distribution bounded by the closed interval between $a$ and $b$ is denoted by \(\mathcal{U}_{[a, b]}\). The angle of a complex scalar or vector is denoted by $\angle$. The operator $\diag \left(\cdot\right)$ is applied in two ways, when operating on a vector it yields a matrix with the input vector on the main diagonal and zeros elsewhere. When operating on a matrix $\diag \left(\cdot\right)$ returns the main diagonal entries as a vector. The standard complex normal (Gaussian) distribution with mean $\mu$, standard deviation $\sigma$ is denoted by $\mathcal{C}\mathcal{N}\left(\mu,\sigma^2\right)$. %The identity matrix $\matr{I}_n$ is a $n\times n$ square matrix with ones on the main diagonal and zeros elsewhere.   



==> rev/before-pruning-for-wcnc/Section/System_Model.tex <==
\section{System Model}
\label{section:system_model}

There is a total of $K$ single-antenna devices and a total of $M$ co-located \gls{bs} antennas. The set of active users trying to access the network is denoted by $\mathcal{K}_a$, with $|\mathcal{K}_a|\leq K$. To access the network, each active device $k\in\mathcal{K}_a$ sends a unique, non-orthogonal preamble of length $T$, known to the network. The pilot symbol of the preamble sent by device $k$ at pilot symbol $t$ is denoted by $s_{k,t}$. The channel vector between the receive antenna $m$ and user $k$ is denoted by $h_{k,m}\in \mathbb{C}$, and is considered fixed over the preamble duration. The received symbol at the $m$-th \gls{bs} antenna at time $t$ is
\begin{align}\label{eq:received_symbol}
    {y}_{t,m}=\sum_{k=0}^{K-1}{h}_{k,m} s_{k,t} \gamma_k + {w}_{t,m}, %\quad m=0,...,M-1,\ t=0,...,T-1,
\end{align}
where $\gamma_k$ is an unknown complex scalar and ${w}_{t,m}\in \mathbb{C}$ is \gls{iid} \gls{zmcscg} noise with variance $\sigma^2$. The unknown complex scalar $\gamma_k$ can be developed as
\begin{align}\label{eq:definition_gamma_k}
    \gamma_k= \sqrt{\rho_k} a_k e^{j\phi_k}, 
\end{align} 
where $\rho_k \in \mathbb{R}^+$ is the transmit power of device $k$, $a_k \in \left\{0,1\right\}$ is the device activity and $\phi_k$ models a potential phase offset.  This offset $\phi_k$ can account for a \gls{cfo}, where the phase is considered constant over the preamble duration. By assuming that all \(M\) antennas are perfectly synchronized, this offset is only dependent on the device. In case the device is inactive, $\gamma_k$ will be zero. We will introduce the term \textit{activity indicator} to denote $\gamma_k$.

Let us consider that the \gls{bs} knows a part of the \gls{csi}, \textit{i.e.}, ${g}_{k,m}$ in
\begin{align}\label{eq:prior_CSI_channel_model}
{h}_{k,m}={g}_{k,m}+ \lambda_k \epsilon_{k,m}, %\quad m=0,...,M-1,\ k=0,...,K-1, 
\end{align}
where $\epsilon_{k,m}$ are \gls{iid} \gls{zmcscg} variables with unit variance, and $\lambda_k \in \mathbb{R}^+$ models the unknown part of the \gls{csi}. The large-scale fading coefficient of user $k$ is $\beta_k  = \mathbb{E}(\norm{\vect{h}_k}^2/M) =\norm{\vect{g}_k}^2/M+\lambda_k^2$. The factor $\lambda_k$ models the quality of the known \gls{csi}. Hence, it quantifies the correlation of the actual channel ${h}_{k,m}$ to the known partial \gls{csi} ${g}_{k,m}$. In the extreme case with $\lambda_k=0$, the \gls{csi} is perfectly known and there is no uncertainty left, as was studied in~\cite{callebaut2021grant}. This could be the case in a fully static environment and if the \gls{csi} estimates are noiseless. However, for a realistic \gls{iot} scenario, even for static devices, \gls{csi} is not perfect due to i) environment dynamics and ii) noisy estimates. The parameter $\lambda_k$ then quantifies this imperfection. It is here assumed to be known\footnote{It could be set to a certain value depending on the user activity profile and/or tracked for each user over time.}. Another extreme case, as considered in \cite{GanesanTCOM,FenglerTIT}, is obtained when ${g}_{k,m}={0}, \forall m$, implying that only the large scale fading coefficient of user $k$ is known, \textit{i.e.}, $\lambda_k=\sqrt{\beta_k}$.



==> rev/before-pruning-for-wcnc/abbr.tex <==
\newacronym{bs}{BS}{base station}
\newacronym{pa}{PA}{power amplifier}
\newacronym{sdr}{SDR}{signal-to-distortion ratio}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{sndr}{SNDR}{signal-to-noise-and-distortion ratio}
\newacronym{snidr}{SNIDR}{signal-to-noise-and-interference-and-distortion ratio}
\newacronym{los}{LOS}{line-of-sight}
\newacronym{z3ro}{Z3RO}{zero third-order distortion}
\newacronym{mimo}{MIMO}{multiple input multiple output}
\newacronym{mrt}{MRT}{maximum ratio transmission}
\newacronym{dpd}{DPD}{digital pre-distortion}
\newacronym{nnls}{NNLS}{non-negative least-squares}
\newacronym{ula}{ULA}{uniform linear array}
\newacronym{embb}{eMBB}{enhanced mobile broadband}
\newacronym{urllc}{URLLC}{ultra reliable low latency communication}
\newacronym{mmtc}{mMTC}{massive machine-type communication}
\newacronym{psd}{PSD}{power spectral density}
\newacronym{aclr}{ACLR}{adjacent channel leakage ratio}
\newacronym{cpu}{CPU}{central processing unit}
\newacronym{iid}{i.i.d.}{independently and identically distributed}
\newacronym{ue}{UE}{user equipment}
\newacronym{nlos}{NLoS}{non-line-of-sight}
\newacronym{hpbm}{HPBM}{half power beam width}
\newacronym{rts}{RTS}{ray tracing simulator}
\newacronym{ag}{AG}{array gain}
\newacronym{arp}{ARP}{Antenna Reference Point}
\newacronym{ecdf}{eCDF}{Empirical Cumulative Distribution Function}
\newacronym{evm}{EVM}{Error Vector Magnitude}
\newacronym{fft}{FFT}{fast Fourier transform}
\newacronym{ib}{IB}{in-band}
\newacronym{im}{IM}{intermodulation}
\newacronym{mf}{MF}{matched filtering}
\newacronym{mr}{MR}{maximum ratio}
\newacronym{ofdm}{OFDM}{orthogonal frequency division multiplexing}
\newacronym{oob}{OOB}{out-of-band}
\newacronym{papr}{PAPR}{Peak-to-Average Power Ratio}
\newacronym{rx}{RX}{Receiver}
\newacronym{trp}{TRP}{Transmission Reception Point}
\newacronym{tx}{TX}{transmitter}
\newacronym{zf}{ZF}{zero forcing}
\newacronym{dl}{DL}{downlink}
\newacronym{rzf}{RZF}{regularized zero forcing}
\newacronym{slc}{SLC}{spatial leakage suppression}
\newacronym{kpi}{KPI}{key performance indicator}
\newacronym{awgn}{AWGN}{additive white gaussian noise}
\newacronym{qam}{QAM}{quadrature amplitude modulation}

\newacronym{zmcscg}{ZMCSCG}{zero mean circularly symmetric complex Gaussian}

\newacronym{ap}{AP}{access point}
\newacronym{cfo}{CFO}{carrier frequency offset}
\newacronym{csi}{CSI}{channel state information}
\newacronym{iot}{IoT}{Internet-of-Things}
\newacronym{lmmse}{LMMSE}{linear minimum mean squared estimator}

\newacronym{llh}{LLH}{log-likelihood}
\newacronym{lorawan}{LoRaWAN}{long-range wide-area network}
\newacronym{ls}{LS}{least squares}

% \newacronym{lorawan}{LoRaWAN}{long-range wide-area network}
% \newacronym{lora}{LoRa}{long range}
% \newacronym{css}{CSS}{chirp spread spectrum}
% \newacronym{lpwan}{LPWAN}{low-power wide-area network}
% \newacronym{fsk}{FSK}{frequency shift keying}
% \newacronym{adr}{ADR}{adaptive data rate}
% \newacronym{mac}{MAC}{medium access control}
% \newacronym{abp}{ABP}{activation-by-personalisation}
% \newacronym{otaa}{OTAA}{over-the-air activation}
% \newacronym{api}{API}{application programming interface}
% \newacronym{aes}{AES}{advanced encryption standard}
% \newacronym{ldo}{LDO}{low-dropout regulator}
% \newacronym{ide}{IDE}{integrated development environment}
% \newacronym{sf}{SF}{spreading factor}
% \newacronym{rf}{RF}{radio frequency}
% \newacronym[plural=PAs,firstplural=power amplifiers (PAs)]{pa}{PA}{power amplifier}
% \newacronym{bw}{BW}{bandwidth}
% \newacronym{mcu}{MCU}{microcontroller unit}
% \newacronym{spi}{SPI}{serial peripheral interface}
% \newacronym{los}{LoS}{line-of-sight}
% \newacronym{kpi}{KPI}{key performance indicator}
% \newacronym{gprs}{GPRS}{general packet radio services}
% \newacronym{egprs}{EGPRS}{enhanced data rates for GSM evolution}
% \newacronym{nbiot}{NB-IoT}{Narrowband IoT}
% \newacronym{lte}{LTE}{long term evolution}
% \newacronym{lpwa}{LPWA}{low-power wide-area}
% %\newacronym{nb}{NB}{narrowband}
% \newacronym{m2m}{M2M}{machine-to-machine}
% \newacronym{cbm}{CBM}{condition based maintenance}
% \newacronym{ai}{AI}{artificial intelligence}
% \newacronym{edrx}{eDRX}{extended discontinuous reception mode}
% \newacronym{drx}{DRX}{discontinuous reception mode}
% \newacronym{psm}{PSM}{power saving mode}
% \newacronym{gps}{GPS}{global positioning system}
% \newacronym{ptw}{PTW}{paging time window}
% \newacronym{tau}{TAU}{tracking area update}
% \newacronym{mtc}{MTC}{machine-type communication}
% \newacronym{ue}{UE}{user equipment}
% \newacronym{cdrx}{cDRX}{connected mode DRX}
% \newacronym{3gpp}{3GPP}{3rd generation partnership project}
% \newacronym{gsm}{GSM}{global system for mobile communications}
% \newacronym{prbs}{PRBs}{physical resource blocks}
% \newacronym{mcl}{MCL}{maximum coupling loss}
% \newacronym{ce}{CE}{coverage enhancement}
% \newacronym{rsrp}{RSRP}{reference signals received power}
% \newacronym{rtc}{RTC}{real time clock}
% \newacronym{ism}{ISM}{industrial, scientific and medical}
% \newacronym{mmtc}{MMTC}{massive machine type communication}
% \newacronym{scfdma}{SC-FDMA}{single-carrier frequency division multiple access}
% \newacronym{udp}{UDP}{user datagram protocol}
% \newacronym{snr}{SNR}{signal-to-noise ratio}
% \newacronym{sinr}{SINR}{signal-to-interference-plus-noise ratio}
% \newacronym{der}{DER}{data extraction rate}
% \newacronym{dr}{DR}{data rate}
% \newacronym{p2p}{P2P}{point-to-point}
% \newacronym{rss}{RSS}{received signal strength}
% \newacronym{erp}{ERP}{effective radiated power}
% \newacronym{lbt}{LBT}{listen before talk}
% \newacronym{afa}{AFA}{adaptive frequency agility}
% \newacronym{pdr}{PDR}{packet delivery ratio}
% \newacronym{pl}{PL}{path loss}
\newacronym{ml}{ML}{maximum-likelihood}
% \newacronym{ols}{OLS}{ordinary least squares}
% \newacronym{cdf}{CDF}{cumulative distribution function}
% \newacronym{pdf}{PDF}{probability density function}
% \newacronym{cobyla}{COBYLA}{constrained optimization by linear approximation}
% \newacronym{per}{PER}{packet error rate}
% \newacronym{mae}{MAE}{mean absolute error}
% \newacronym{rmse}{RMSE}{root mean square error}
% \newacronym{cr}{CR}{coding rate}
% \newacronym{ofdm}{OFDM}{orthogonal frequency-division multiplexing}
% \newacronym{ofdma}{OFDMA}{orthogonal frequency division multiple access}
% \newacronym{qos}{QoS}{quality of service}
% \newacronym{ra}{RA}{random access}
% \newacronym{rar}{RAR}{random access response}
% \newacronym{ttm}{TTM}{time to market}
% \newacronym{cots}{COTS}{commercial off-the-shelf}
% \newacronym{multi-rat}{multi-RAT}{multiple radio access technology}
% \newacronym{lib}{LIB}{lithium-ion battery}
% \newacronym{lipo}{LIPO}{lithium polymer}
% \newacronym{msk}{MSK}{minimum-shift keying}
% \newacronym{qam}{QAM}{quadrature amplitude modulation}
% \newacronym{em}{EM}{electromagnetic}
% \newacronym{papr}{PAPR}{peak-to-average power ratio}
% \newacronym{pv}{PV}{photovoltaic}
% \newacronym{dbpsk}{DBPSK}{differential binary phase shift keying}
% \newacronym{bpsk}{BPSK}{binary phase shift keying}
% \newacronym{qpsk}{QPSK}{quadrature phase shift keying}
% \newacronym{pmu}{PMU}{power management unit}
% \newacronym{bod}{BOD}{brown-out detection}
% \newacronym{ram}{RAM}{random-access memory}
% \newacronym{io}{IO}{input/output}
% \newacronym{fram}{FRAM}{ferroelectric random access memory}
% \newacronym{fft}{FFT}{fast fourier transform}
% \newacronym{tpms}{TPMS}{tire-pressure monitoring system}
% \newacronym{phy}{PHY}{physical}
% % \newacronym{lco}{LCO}{Lithium Cobalt Oxide}
% % \newacronym{lto}{LTO}{Lithium Titanium Oxide}
% % \newacronym{lic}{LIC}{Lithium-ion Capacitor}
% % \newacronym{alk}{ALK}{Alkaline}
% % \newacronym{ltc}{LTC}{Lithium Thionyl Chloride}
% % \newacronym{lmd}{LMD}{Lithium Manganese Dioxide}
% % \newacronym{lid}{LID}{Lithium Iron Disulfide}
% \newacronym{pc}{PC}{lithium poly carbon}
% \newacronym{edlc}{EDLC}{electric double-layer capacitor}
% \newacronym{cmos}{CMOS}{complementary metal-oxide-semiconductor}
% \newacronym{soc}{SoC}{state of charge}
% \newacronym{SoC}{SOC}{system on chip}
% \newacronym{imu}{IMU}{inertial measurement unit}
% \newacronym{agps}{A-GPS}{assisted global positioning system}
% \newacronym{i2c}{I2C}{inter-integrated circuit}
% \newacronym{adc}{ADC}{analog-to-digital converter}
% \newacronym{led}{LED}{light emitting diode}
% \newacronym{gpio}{GPIO}{general-purpose input/output}
% \newacronym{pcb}{PCB}{printed circuit board}
% \newacronym{prs}{PRS}{peripheral reflex system}
% \newacronym{sha}{SHA}{secure hash algorithm}
% \newacronym{ecc}{ECC}{elliptic-curve cryptography}
% \newacronym[plural=UVs,firstplural=Unmanned Vehicles]{uv}{UV}{unmanned vehicle}
% \newacronym{voc}{VOC}{voltatile organic compound}
% \newacronym{iaq}{IAQ}{indoor air quality}
% \newacronym{gnss}{GNSS}{global navigation satellite system}
% \newacronym{ttff}{TTFF}{time to first fix}
% \newacronym{pll}{PLL}{phase-locked loop}
% \newacronym{crc}{CRC}{cycle redundancy check}
% \newacronym{dma}{DMA}{direct memory access}
% \newacronym{cpu}{CPU}{central processing unit}
% \newacronym{dmac}{DMAC}{direct memory access controller}
% \newacronym{dram}{DRAM}{dynamic random-access memory}
% \newacronym{mppt}{MPPT}{maximum power point tracking}
% \newacronym{sram}{SRAM}{static random-access memory}
% \newacronym{uart}{UART}{universal asynchronous receiver/transmitter}
% \newacronym{awgn}{AWGN}{additive white gaussian noise}
% \newacronym{at}{AT}{ATtention}
% \newacronym{pse}{PSE}{power sourcing equipment}
% \newacronym{pd}{PD}{powered device}
% \newacronym{usrp}{USRP}{universal software radio peripheral}
% \newacronym{rpi}{RPi}{Raspberry Pi}
% \newacronym{poe}{PoE}{power over ethernet}
% \newacronym{ptp}{PTP}{precision time protocol}
% \newacronym{vlc}{VLC}{visible light communication}
% \newacronym{vlp}{VLP}{visible light positioning}
% \newacronym{tsn}{TSN}{time-sensitive networking}
% \newacronym{sdr}{SDR}{software-defined radio}
% \newacronym{pps}{PPS}{pulse per second}
% \newacronym{gpclk}{GPCLK}{general purpose clock}
% \newacronym{ros}{ROS}{robot operating system}
% \newacronym{tof}{ToF}{time-of-flight}
% \newacronym{ntp}{NTP}{network time protocol}
% \newacronym{uhd}{UHD}{USRP hardware driver}
% \newacronym{os}{OS}{operating system}
% \newacronym{hat}{HAT}{hardware attached on top}
% \newacronym{gpu}{GPU}{graphical processing unit}
% \newacronym{if}{IF}{intermediate frequency}
% \newacronym{fpga}{FPGA}{field-programmable gate array}
% \newacronym{rfic}{RFIC}{radio-frequency integrated circuit}
% \newacronym{ssd}{SSD}{solid state drive}
% \newacronym{mimo}{MIMO}{multiple input multiple output}
% \newacronym{mumimo}{MU-MIMO}{multiuser MIMO}
% \newacronym[plural=BSs,firstplural=base stations (BSs)]{bs}{BS}{base station}
% \newacronym{ib}{IB}{in-band}
% \newacronym{oob}{OOB}{out-of-band}
% \newacronym{rts}{RTS}{ray-tracing simulator}
% \newacronym{nlos}{NLoS}{non line-of-sight}
% \newacronym{evm}{EVM}{error vector magnitude}
% \newacronym{mr}{MR}{maximum ratio}
% \newacronym{zf}{ZF}{zero forcing}
% \newacronym{aclr}{ACLR}{adjacent channel leakage power ratio}
% \newacronym{bo}{BO}{back-off}
% \newacronym{psd}{PSD}{power spectral density}
% \newacronym{im}{IM}{intermodulation}
% \newacronym{arp}{ARP}{antenna reference point}
% \newacronym{ag}{AG}{array gain}
% \newacronym{ula}{ULA}{uniform linear array}
% \newacronym{rrc}{RRC}{radio resource connection}
% \newacronym{ecdf}{eCDF}{empirical cumulative distribution function}
% %\newacronym{sdr_distortion}{SDR}{Signal-to-Distortion Ratio}
% \newacronym{iid}{i.i.d.}{independently and identically distributed}
% \newacronym{hpbm}{HPBM}{half-power beam width}
% \newacronym{mf}{MF}{matched filtering}
% \newacronym{mrt}{MRT}{maximum ratio transmission}
% \newacronym{rx}{RX}{receiver}
% \newacronym{trp}{TRP}{transmission reception point}
% \newacronym{tx}{TX}{transmitter}
% \newacronym{dl}{DL}{downlink}
% \newacronym{ul}{UL}{uplink}
% \newacronym{rzf}{RZF}{regularized zero forcing}
% \newacronym{enb}{eNB}{evolved Node B}
% \newacronym{rat}{RAT}{radio access technology}
% \newacronym{dsp}{DSP}{digital signal processing}
% \newacronym{tdma}{TDMA}{time-devision multiple-access}
% \newacronym{ota}{OTA}{over-the-air}
% %\newacronym{ula}{ULA}{Uniform Linear Array}
% \newacronym{ura}{URA}{uniform rectangular array}
% \newacronym{dsss}{DSSS}{direct-sequence spread spectrum}
% \newacronym{tdd}{TDD}{time-division duplexing}
% \newacronym{fdd}{FDD}{frequency-division duplexing}
% \newacronym{omp}{OMP}{orthogonal matching pursuit}
% \newacronym{sucre}{SUCRe}{strongest-user collision resolution}
\newacronym{mse}{MSE}{mean-square error}
% \newacronym{roc}{ROC}{receiver operating characteristic}
% \newacronym{dop}{DOP}{dilution of precision}
% %\newacronym{ml}{ML}{maximum likelihood}
% \newacronym{nnls}{NNLS}{non-negative least squares}
% \newacronym{mmv-amp}{MMV-AMP}{multiple measurement vector - approximated massage passing}
